LLM Agents Do Not Replicate Human Market Traders: Evidence From Experimental Finance

This paper explores how Large Language Models (LLMs) behave in a classic experimental finance paradigm widely known for eliciting bubbles and crashes in human participants. We adapt an established trading design, where traders buy and sell a risky asset with a known fundamental value, and introduce several LLM-based agents, both in single-model markets (all traders are instances of the same LLM) and in mixed-model "battle royale" settings (multiple LLMs competing in the same market). Our findings reveal that LLMs generally exhibit a "textbook-rational" approach, pricing the asset near its fundamental value, and show only a muted tendency toward bubble formation. Further analyses indicate that LLM-based agents display less trading strategy variance in contrast to humans. Taken together, these results highlight the risk of relying on LLM-only data to replicate human-driven market phenomena, as key behavioral features, such as large emergent bubbles, were not robustly reproduced. While LLMs clearly possess the capacity for strategic decision-making, their relative consistency and rationality suggest that they do not accurately mimic human market dynamics.

==> tex/word_count_compare_10.tex <==
\begin{tabular}{llrrlrr}
\toprule
 & \multicolumn{3}{c}{Human} & \multicolumn{3}{c}{LLM-Agent} \\
 & Word & Count & Freq & Word & Count & Freq \\
Rank &  &  &  &  &  &  \\
\midrule
1 & \textbf{sell} & 230 & 5.60\% & \textbf{price} & 88707 & 6.04\% \\
2 & \textbf{buy} & 202 & 4.92\% & \textbf{market} & 63445 & 4.32\% \\
3 & \textbf{stock} & 177 & 4.31\% & \textbf{buy} & 38996 & 2.66\% \\
4 & \textbf{price} & 141 & 3.43\% & \textbf{sell} & 38141 & 2.60\% \\
5 & tried & 129 & 3.14\% & orders & 31335 & 2.14\% \\
6 & \textbf{market} & 79 & 1.92\% & round & 28385 & 1.93\% \\
7 & low & 75 & 1.83\% & \textbf{stock} & 28130 & 1.92\% \\
8 & high & 70 & 1.70\% & cash & 26469 & 1.80\% \\
9 & would & 57 & 1.39\% & continue & 23318 & 1.59\% \\
10 & interest & 53 & 1.29\% & adjust & 19250 & 1.31\% \\
\bottomrule
\end{tabular}

